Partial DNA Assembly: A Rate-Distortion Perspective

Earlier formulations of the DNA assembly problem were all in the context of perfect assembly; i.e., given a set of reads from a long genome sequence, is it possible to perfectly reconstruct the original sequence? In practice, however, it is very often the case that the read data is not sufficiently rich to permit unambiguous reconstruction of the original sequence. While a natural generalization of the perfect assembly formulation to these cases would be to consider a rate-distortion framework, partial assemblies are usually represented in terms of an assembly graph, making the definition of a distortion measure challenging. In this work, we introduce a distortion function for assembly graphs that can be understood as the logarithm of the number of Eulerian cycles in the assembly graph, each of which correspond to a candidate assembly that could have generated the observed reads. We also introduce an algorithm for the construction of an assembly graph and analyze its performance on real genomes.

==> distortion.tex <==
% !TEX root = partial01-12.tex


One of the issues with defining the distortion as the log of the number of Eulerian cycles in the resulting graph is that the sequence graph constructed is in general not Eulerian (it is expected to contain a Chinese cycle, but the multiplicities are not known).
One way to go around that is to consider the multiplicities induced on the sequence graph by the true sequence $\s$.
While that is not known from the point of view of the assembler, it can be used in the computation of the distortion metric.

\begin{definition}
Suppose $G = (V,E,\ch)$ is a sufficient sequence graph, and suppose $c_\s$ is a Chinese cycle in $G$ corresponding to the sequence $\s$.
Let $G[{\s}]$ be the multi-graph obtained by setting the multiplicity of edge $e$ to be the number of times $c_\s$ traverses $e$.
We define the distortion of a sequence graph $G$ as
\aln{
D(G,\s) \defi \left\{ 
\begin{array}{ll}
\log \ec(G[\s]) & \text{ if $G$ is a sufficient sequence graph} \\
\log \ec(G_1[\s]) +1 & \text{ otherwise} 
\end{array} 
\right.\label{eq:dist_defn}
}
where $\ec(G)$ is the number of distinct Eulerian cycles in $G[\s]$, and $G_1$ is the trivial sequence graph illustrated in Fig.~\ref{trivialfig}.
Two Eulerian cycles are distinct if they define distinct sequences (up to cyclic shifts).
\end{definition}

\begin{figure}[h]
\centering
\includegraphics[width = 0.32\linewidth]{trivialgraph}
\caption{The trivial sequence graph $G_1$ is always sufficient.} 
\label{trivialfig}
\end{figure}

How do we prove that \Cref{alg:greedyalg} has good distortion properties?
A reasonable bound on the distortion can be obtained as follows.


%\begin{definition}
%A triple repeat is said to be super-bridged if the maximal repeats obtained by considering each pair of copies are all doubly-bridged.
%\end{definition}

\begin{definition}
Two maximal repeats $\s[a_1: a_1+\ell]$, $\s[a_2: a_2+\ell]$ and $\s[b_1: b_1+k]$, $\s[b_2: b_2+k]$ are said to be linked if $a_2 < b_1 \leq a_2 + \ell + 1$.
In this case, we call $a_2 + \ell + 1-b_1$ the link length.
\end{definition}

\begin{theorem} \label{distthm}
Suppose that the set of reads $\Rs$ from the sequence $\s$ satisfies the following conditions:
\begin{enumerate}
\item each triple repeat is either all-bridged or all-unbridged,
\item all maximal repeats of length $\leq k$ are doubly-bridged,
\item for all pairs of linked repeats with link length $\leq k$, at least one is doubly-bridged.
\end{enumerate}
% all triple repeats of length $\leq k$ are super-bridged.
Then the sufficient sequence graph $G$ produced by \Cref{alg:greedyalg} has a distortion satisfying
\aln{
D(G,\s) \leq D(\dbg_k(\s),\s),
}
where $\dbg_k(\s)$ is the de Bruijn graph of order $k$ of $\s$.
\end{theorem}

\obs 
There is a slight issue with the statement above because $\dbg_k(\s)$ is not a sequence graph in the sense of Definition 1.
However, one can still think of $\ec(G_k[\s])$ as the number of distinct assemblies implied by the de Bruijn graph of order $k$.
\vspace{4mm}


In the context of a sequence graph, the circular genome $\s$ can be represented as a cycle graph $\G = (\V,\E,\ch)$ with nodes $\V = \{1,...,G\}$ and edges $\E = \{(1,2),...,(G-1,G),(G,1)\}$ and $\ch(i,i+1) = \s[i]$.
This can be thought of as a canonical sufficient sequence graph and it achieves $D(\G,\s) = 0$, although we point out that other assembly graphs may achieve zero distortion as well.


A repeat of length $\ell$ in $\s$ corresponds to two $(\ell+1)$-node paths on $\G$, say $[a : a+\ell]$ and $[b : b+\ell]$.
One can define a new sequence graph by taking $\G$ and contracting the paths $[a : a+\ell]$ and $[b : b+\ell]$; i.e., merging the corresponding nodes and edges.
Notice that since the edges $(a,a+1),...,(a+\ell-1,a+\ell)$ and $(b,b+1),...,(b+\ell-1,b+\ell)$ correspond to the same symbols from $\Sigma$, contracting the two paths is a well-defined operation.
In general, for a set of repeats 
\aln{
\T = \left\{ \left( [a_1 : a_1 + \ell_1], [b_1 : b_1 + \ell_1 ]\right), ..., \left( [a_m : a_m + \ell_m], [b_m : b_m + \ell_m ]\right) \right\},
}
one can consider the sequence graph $\G_\T$ obtained by contracting the paths $[a_i: a_i+\ell_i]$ and $[b_i : b_i+\ell_i]$ corresponding to each repeat.
It is straightforward to see that the order in which these merging operations are carried out does not affect the resulting graph.
%For the sake of formalism, we can define $\G_\T$ as follows.
%First we define the set of undirected edges
%\aln{
%\W = \left\{ (a_i + t, b_i+t) \, : \, 1 \leq i \leq m, \, 0 \leq t < \ell_i \right\}.
%}
%The connected components of $(\V,\W)$ define the node set of $\G_\T$.
%The edge set 
%
%
%We then define another set of undirected edges
%\aln{
%\W' = \left\{ (a_i + t, b_i+t) \, : \, 1 \leq i \leq m, \, 0 \leq t < \ell_i - 1  \right\}.
%}
%
%
%As we formally explain next, the order in which these merging operations are performed does not alter the result.
%To see this, consider defining an undirected graph with node set $\V$ and edge set
%\aln{
%\W = \left\{ (a_i + t, b_i+t) \, : \, 1 \leq i \leq m, \, 0 \leq t < \ell_i \right\}.
%}
%The edges in $\W$ correspond to two nodes from $\V$ that will be merged when we perform the contraction operations to obtain $\G_\T$.
%It is then clear that the connected components in $(\V,\W)$ correspond to the resulting nodes of $\G_\T$, regardless of the order of operations.
%Moreover, 
%
%Regardless of the order in which we perform the merging operations to obtain $\G_\T$, the node set of $\G_\T$
%In addition, we point out the de Bruijn graph of order $k$ can be thought of as $\G_{\T_k}$, where $\T_k$ is the set of all maximal repeats in $\s$ of length at least $k$.
%
%
%
%In general, another sufficient sequence graph $G = (V,E,\ch)$ can be understood as the canonical graph $\G$ after certain sets of nodes have been contracted.
%More precisely, for 
%On this graph, a repeat of length $\ell$ corresponds to a path with $\ell+1$ nodes and $\ell$ edges.
Given the set of reads $\Rs$ one can then define the set $\U$ of maximal non-doubly-bridged repeats.
%\aln{
%\U = \left\{ \left( [a_1 : a_1 + \ell_1], [b_1 : b_1 + \ell_1 ]\right), ..., \left( [a_m : a_m + \ell_m], [b_m : b_m + \ell_m ]\right) \right\},
%}
%where $\ell_i$ is the length (in bases) of the $i$th repeat in the set.
As described above, this set of repeats defines a sequence graph $\G_\U$ where each repeat in $\U$ is merged.
As it turns out, we will show that the when the conditions in \Cref{distthm} are satisfied, the sequence graph produced by \Cref{alg:greedyalg} has a distortion that is upper bounded by $D(\G_\U,\s)$.


%The set $\U$ determines an undirected graph with node set $\V$ and edge set
%\aln{
%\W = \left\{ (a_i + t, b_i+t) \, : \, 1 \leq i \leq m, \, 0 \leq t < \ell_i \right\}.
%}
%One can then define a sequence graph $G_\U$ by taking the cycle graph $(\V,\E)$ and contracting the nodes in each connected component of $(\V,\W)$.
%Intuitively, this can be understood as collapsing the segments in $(\V,\E)$ corresponding to repeats in $\U$.
%   creating one node for each connected component of $(\cG,\cE)$ and, for $(j,j+1)$, $1 \leq j \leq G-1$, we place a directed edge between the node corresponding to the connected component in $(\cG,\cE)$ containing $j$ and the connected component in  $(\cG,\cE)$ containing $j+1$.

%Next we require the following lemma regarding the graph produced by the algorithm:
%
%
%\begin{lemma} \label{overlaplem}
%If a maximal repeat $[a : a + \ell]$, $[b : b + \ell ]$ is doubly-bridged by $\Rs$, then the sequence graph produced by \Cref{greedyalg} contains two node-disjoint paths (of length $\ell+1$) corresponding to each of the two copies.
%\end{lemma}



First we consider the initial sequence graph in \Cref{alg:greedyalg} (disjoint paths for each read), and consider assigning a number from $\V$ to each node according to the position in $\s$ the read comes from (or a set of numbers, in case the read comes from inside a repeat).
As the algorithm progresses, and nodes are merged, suppose we take the union of the set of numbers at the merged nodes.
If the conditions  of \Cref{correctthm} are satisfied, the Chinese cycle corresponding to $\s$ in the final sequence graph will be determined by following the numbers in $\V  = \{1,...,G\}$ {\bf (maybe we need a slight strengthening of the statement of Theorem 1)}.
%The set of numbers associated to each node of this final graph defines a partition of $\V= \{1,...,G\}$.
We claim that every time we merge two nodes that have distinct labels (and we take the union of the labels), we must be merging nodes that are merged in $\G_\U$.
To see this we notice that, at each merging operation of \Cref{alg:greedyalg}, we can only merge two paths that do not correspond to the same segment in $\s$ if they correspond to a repeat that is not doubly-bridged.
%Therefore, we may only merge two nodes if they correspond to nodes in the same connected component of $(\V,\W)$, which implies that the resulting partition is finer than (or equal to) the partition implied by $(\V,\W)$.
Therefore, $\G_\U$ is either equal to the output of \Cref{alg:greedyalg} or can be obtained by performing further node contractions.
This implies that the distortions of these two assemblies are related by 
\aln{
D(G,\s) \leq D(G_\U,\s).
}

%We claim that this partition of $\V$ must be a refinement of the partition defined by the connected components of $(\V,\W)$.
%To see this we notice that, at each merging operation of \Cref{alg:greedyalg}, we can only merge two paths that do not correspond to the same segment in $\s$ if they correspond to a repeat that is not doubly-bridged.
%Therefore, we may only merge two nodes if they correspond to nodes in the same connected component of $(\V,\W)$, which implies that the resulting partition is finer than (or equal to) the partition implied by $(\V,\W)$.
%This implies that the distortions of these two assemblies are related by 
%\aln{
%D(G,\s) \leq D(G_\U,\s).
%}

Next we need to bound $D(G_\U,\s)$.
To do that, we claim that any (directed) $k$-edge path in $G_\U$ starting at a node $v_1$ with $\din(v_1) > 1$ and visiting nodes $v_2,v_3,...,v_{k+1}$ must have the property that $\dout(v_i) = 1$ for $i=1,...,k+1$.
%
%
%must have the property that either $\din(v_i) = 1$ for $i=1,...,k$ or $\dout(v_i) = 1$ for $i=1,...,k$.
To see this we first notice that a node $v$ in $G_\U$ can only have $\din(v) > 1$ if it is the starting node of some repeat in $\U$.
Similarly, a node $v$ can only have $\dout(v) > 1$ if it is the ending node of some repeat in $\U$.
%Consider a path $(v_1,...,v_k)$ in $G_\U$ starting at a node $v_1$ with $\din(v_1) > 1$, and 
Suppose by contradiction that $\dout(v_i) > 1$ for some $i \leq k+1$, and let $m$ be the first such index.
Clearly, when the Chinese cycle reaches $v_1$, it must traverse the edges in the path until $v_m$, and
the path $v_1,...,v_m$ must correspond to the beginning of the repeat started at $v_1$.
Since $\dout(v_m)>1$, $v_m$ corresponds to the end of a repeat.
This means that $\s$ has two linked repeats in $\U$ (hence not doubly bridged) with a junction length  $m-1 \leq k$. 
But this is a contradiction to the assumption that, for every pair of linked repeats with link lengths $\leq k$, at least one is doubly bridged.

Next we claim that every $k$-edge path in $G_\U$ must be fully traversed by the Chinese cycle corresponding to $\s$.
From the previous argument, 
we know that the nodes in $(v_1,...,v_{k+1})$ with $\dout(v_i) > 1$ must precede the nodes with $\din(v_i) > 1$; i.e., there exists a $q \in \{1,...,k\}$ such that $\din(v_i) = 1$ for $i=1,...,q$ and $\dout(v_i) = 1$ for $i=q+1,...,k+1$.
Since the Chinese cycle must visit node $v_q$, it must arrive there through the path $(v_1,...,v_q)$.
Since the cycle must continue after $v_q$, it needs to traverse the remainder of the path $(v_{q+1},...,v_{k+1})$.
We conclude that any $k$-mer in $G_\U$ must be a true $k$-mer of $\s$.
Therefore, any Chinese cycle in $G_\U$ must correspond to a Chinese cycle in $\dbg_k(\s)$.
In particular, any Eulerian cycle in $G_\U[\s]$ must correspond to an Eulerian cycle in $\dbg_k(\s)$ {\bf (is this clear?)}, and we must have
\aln{
D(G_\U,\s) \leq D(\dbg_k(\s),\s).
}



